Achieving State Machine Replication without Honest Players

Existing standards for player characterisation in tokenised state machine replication protocols depend on honest players who will always follow the protocol, regardless of possible token increases for deviating. Given the ever-increasing market capitalisation of these tokenised protocols, honesty is becoming more expensive and more unrealistic. As such, this out-dated player characterisation must be removed to provide true guarantees of safety and liveness in a major stride towards universal trust in state machine replication protocols and a new scale of adoption. As all current state machine replication protocols are built on these legacy standards, it is imperative that a new player model is identified and utilised to reflect the true nature of players in tokenised protocols, now and into the future. To this effect, we propose the ByRa player model for state machine replication protocols. In the ByRa model, players either attempt to maximise their tokenised rewards, or behave adversarially. This merges the fields of game theory and distributed systems, an intersection in which tokenised state machine replication protocols exist, but on which little formalisation has been carried out. In the ByRa model, we identify the properties of strong incentive compatibility in expectation and fairness that all protocols must satisfy in order to achieve state machine replication. We then provide Tenderstake, a protocol which provably satisfies these properties, and by doing so, achieves state machine replication in the ByRa model.

==> Appendices/Proofs.tex <==

\section{Proofs}\label{appendix:proofs}

\begingroup
\def\thetheorem{\ref{lem:dominantXOR}}
\begin{lemma}
    For an SMR protocol $\protocol$, a rational player $\playeri$, any strategy $\strategyi^1 \in \strategySeti$ , and $|\strategySeti|\geq 2$, either $\strategyi^1 \in \strategySetNonDominatedi $ or there is some $ \strategyi^2 \in \strategySetNonDominatedi$ such that $\strategyi^2 \strictlyDominates \strategyi^1$.
\end{lemma}
\endgroup

\addtocounter{theorem}{-1}

\begin{proof}
    We will do this by induction over the cardinalities of $\strategySeti$.
    First we check $| \strategySeti|=2$. If $\strategyi^a$ is in $\strategySetNonDominatedi $, we are finished. Assume otherwise. That is,  $\strategyi^b \strictlyDominates \strategyi^a$, which implies $\strategyi^a \not\strictlyDominates\strategyi^b$, and as such, $\strategyi^b \in \strategySetNonDominatedi $ as required. 
    
    Assume the inductive hypothesis for $| \strategySeti|=k$. 
    
    Now, given this assumption, we must prove our hypothesis holds for $| \strategySeti|=k+1$. Consider a strategy $\strategyi^c \in  \strategySeti$. We need to prove either $\strategyi^c \in \strategySetNonDominatedi$, or there exists $ \, \strategy \in \strategySetNonDominatedi$ with $\strategy \strictlyDominates \strategyi^c$.
    If $\strategyi^c$ is not strictly dominated by any strategy $\strategy \in \strategySeti$, then $\strategyi^c \in \strategySetNonDominatedi$. 
    
    Assume instead there exists some strategy $\strategyi^a \in \strategySeti$, $\strategyi^a \strictlyDominates \strategyi^c$. Consider $Z_i=  \strategySeti \backslash \{ \strategyi^c\}$.
    By the inductive assumption, either $\strategyi^a \in Z_i^\notStrictlyDominated$, or there exists $ \, \strategyi^b \in Z_i^\notStrictlyDominated$ such that $\strategyi^b \strictlyDominates  \strategyi^a$. 
    If $\strategyi^a \in Z_i^\notStrictlyDominated$, then $\strategyi^a \in \strategySetNonDominatedi$, which implies there exists $ \, \strategy \in \strategySetNonDominatedi$ such that $ \strategy \strictlyDominates \strategyi^c$. 
    Otherwise, if $\strategyi^a \not \in Z_i^\notStrictlyDominated$, there exists $ \,  \strategyi^b \in Z_i^\notStrictlyDominated$, with $\strategyi^b \strictlyDominates \strategyi^a$. 
    As $\strategyi^b \strictlyDominates \strategyi^a$, and $\strategyi^a \strictlyDominates \strategyi^c$, this implies $\strategyi^b \strictlyDominates \strategyi^c$. 
    As $\strategyi^b \in Z_i^\notStrictlyDominated$, and $\strategyi^b \strictlyDominates \strategyi^c$, this implies $\strategyi^b \in \strategySetNonDominatedi$. Therefore, there exists $ \,  \strategy \in \strategySetNonDominatedi$ such that $ \strategy \strictlyDominates \strategyi^c$.

\end{proof}


\begingroup
\def\thetheorem{\ref{lem:SICIEiffNSD}}
\begin{lemma}
    For an SMR protocol $\protocol$ and a rational player $\playeri$, $\strategySetNonDominatedi= \{ \strategyProtocol \}$ if and only if $\protocol$ is strong incentive compatible in expectation.
\end{lemma}
\endgroup

\addtocounter{theorem}{-1}

\begin{proof}
    If an SMR protocol $\protocol$ is $\SICIE$, then for any rational player $\playeri$,  $\strategyProtocol$ strictly dominates all other strategies in expectation. From Lemma \ref{lem:dominantXOR}, this implies $\strategySetNonDominatedi= \{\strategyProtocol\}$. 
    
    Now we need to show if  $\strategySetNonDominatedi= \{ \strategyProtocol \}$, then $\protocol$ is $\SICIE$. From Lemma \ref{lem:dominantXOR}, we know for any strategy $\strategyi^a$, either $\strategyi^a \in \strategySetNonDominatedi $ or there is some $ \strategyi^b \in \strategySetNonDominatedi$ such that $\strategyi^b \strictlyDominates \strategyi^a$. As the only strategy in $\strategySetNonDominatedi$ is $ \strategyProtocol$, this implies for any strategy $\strategyi^a \, \notequiv \, \strategyProtocol$, $\strategyProtocol \strictlyDominates \strategyi^a$. This implies $\protocol$ is $\SICIE$, as required. 
\end{proof}

\begingroup
\def\thetheorem{\ref{lem:noHonestInValues}}
\begin{lemma}
    It is not possible to generate a valid deviation proof for an honest player.
\end{lemma}
\endgroup

\addtocounter{theorem}{-1}

\begin{proof}
    A valid deviation proof for some player $\playeri$ must identify a message from $\playeri$ that is invalid according to one of the methods listed in Section \ref{sec:PoD}, which covers all possible message deviations. By definition, honest players follow all protocol rules and only send valid messages. We also know that honest player messages cannot be forged under our threat model assumption regarding unforgeable signatures from Section \ref{sec:ThreatModel}. Furthermore, as $\adversary$ is static, every message signed by a currently honest player must have been generated honestly (by that same player) at some point in the protocol. Therefore, all honest player messages are valid, and as such, no valid proof-of-deviation described in Section \ref{sec:PoD} can be generated for honest players. 
\end{proof}




\begingroup
\def\thetheorem{\ref{lem:boundedDeviatorPot}}
\begin{lemma}
    In any instance of $\protocolName$, $\playeri$ receives less than $\sharei^{\initialisationHeight} \rewardInitial$ in total for identifying deviators from the \textit{adjustForSlashing} function.
\end{lemma}
\endgroup

\addtocounter{theorem}{-1}


\begin{proof}
    We can see that the rewards for deciding on new deviators at height $\blockchainHeight$ are distributed at line \ref{line:splitDeviatorPot}. We will prove that the sum of the rewards distributed by calling line \ref{line:splitDeviatorPot} throughout an instance of $\protocolName$ are less than $\sharei^{\initialisationHeight} \rewardInitial$.
    
    
    Let there be a set of players $\textit{newDevs}^\blockchainHeight$ controlling $\slashedShare$ at height $\blockchainHeight-1$ identified as deviating for the first time in the value at height $\blockchainHeight$. 
    In the \textit{adjustForSlashing} function, this results in $\playeri$'s share being updated according to line \ref{line:adjustShares}, which implies $\shareHi =\frac{\sharei^{\blockchainHeight-1}}{1-\slashedShare}$. Furthermore, letting $\reward^{\blockchainHeight-1}$ be the total reward after deciding on a value at height $\blockchainHeight-1$, the new total reward for height $\blockchainHeight$ is $\reward^\blockchainHeight= (1-\slashedShare) \reward^{\blockchainHeight-1}  $ (line \ref{line:adjustReward}), while the total stake before distributing rewards for height $\blockchainHeight$ is adjusted to $(1-\slashedShare) \stake^{\blockchainHeight-1} $ (line \ref{line:adjustStake}), preserving the total stake of non-deviators. We then have to add the slash bonus of $\sum_{j \in \textit{newDevs}^\blockchainHeight} $ $\textit{Genesis.shares}()[j] \reward^\blockchainHeight$  (line \ref{line:splitDeviatorPot}).

    First observe that:  
    \begin{equation}
    \begin{split}
         \sharei^{\blockchainHeight} \reward^{\blockchainHeight} &= \frac{\sharei^{\blockchainHeight-1}}{1-\slashedShare} (1-\slashedShare) \reward^{\blockchainHeight-1}  \\ 
        &= \sharei^{\blockchainHeight-1}  \reward^{\blockchainHeight-1}.
    \end{split}
    \end{equation}
    
    Secondly, notice that when no new deviators are identified, and \textit{adjustForSlashing} is not called, both $\sharei$ and $\reward_i$ are unchanged from the previous height, as they are only adjusted in \textit{adjustForSlashing}. This means: 
    \begin{equation} \label{eq:ConstantReward}
        \sharei^{\blockchainHeight} \reward^{\blockchainHeight}
        = \sharei^\initialisationHeight \reward^{\initialisationHeight}
        =\sharei^\initialisationHeight \rewardInitial, \ \forall \ \blockchainHeight \geq 1.
    \end{equation}
    
    We know for a set of new deviators $\textit{newDevs}^\blockchainHeight$ at height $\blockchainHeight$, $\playeri$ receives $\sharei^{\blockchainHeight} \reward^{\blockchainHeight} $ $ \sum_{j \in {\textit{newDevs}^\blockchainHeight}} $ $ \textit{Genesis.shares}()[j] $(line \ref{line:splitDeviatorPot}). 
    Furthermore, from Equation \ref{eq:ConstantReward}, we have that  $\sharei^{\blockchainHeight} \reward^{\blockchainHeight}= \sharei^\initialisationHeight $ $ \rewardInitial$ for all $\blockchainHeight \geq 1$. 
    This implies $\playeri$ receives an identifying deviator bonus from \textit{adjustForSlashing} of $\sharei^\initialisationHeight   \rewardInitial \cdot $ $\sum_{j \in {\textit{newDevs}^\blockchainHeight}}$ $ \textit{Genesis.shares}()[j]$ at height $\blockchainHeight$. 
    Summing over all heights up to and including $\blockchainHeight$ gives a total reward of $\sharei^\initialisationHeight $ \\ $  \rewardInitial \cdot \sum^\blockchainHeight_{k=1}  $ $\big( \sum_{j \in {\textit{newDevs}^k}} $ $\textit{Genesis.shares}()[j] \big)$ for identifying deviators through \textit{adjustForSlashing}. 
    
    As $\cup_{1 \leq k\leq \blockchainHeight} {\textit{newDevs}^k} \subset \{1, ..., \numPlayers\}$ for all $\blockchainHeight > 1$, it must be that $\sum^\blockchainHeight_{k=1} \big( \sum_{j \in {\textit{newDevs}^k}} $ $\textit{Genesis.shares}()[j] \big) < 1$ for all $\blockchainHeight > 1$.
    This means the total reward for identifying deviators in $\protocolName$ through the \textit{adjustForSlashing} function is less than $\sharei^\initialisationHeight  \rewardInitial$, as required. 
\end{proof}

\begingroup
\def\thetheorem{\ref{lem:constantReward}}
\begin{lemma}
    In addition to any rewards from the \textit{adjustForSlashing} function, $\playeri$ receives $\sharei^{\initialisationHeight} \rewardInitial$ for every decided value in $\protocolName$.
\end{lemma}
\endgroup

\addtocounter{theorem}{-1}

\begin{proof}
    The only reward received by $\playeri$ not in \textit{adjustForSlashing} is distributed at line \ref{line:addReward}. Letting $\reward^{\blockchainHeight}$ be the total reward distributed at line \ref{line:addReward} for height $\blockchainHeight$, $\playeri$ receives $\sharei^{\blockchainHeight} \reward^{\blockchainHeight}$. We have already seen in Equation \ref{eq:ConstantReward} that $\sharei^{\blockchainHeight} \reward^{\blockchainHeight}= \sharei^\initialisationHeight  \rewardInitial$, for all $\blockchainHeight \geq 1$, which is the required result. 
    
    
\end{proof}


==> Appendices/Quotes.tex <==
\section{Quotes}

\begin{itemize}
    \item \cite{GeneralFrameworkSecurityAnalysisBlockchain}: In the real world, users are not simply honest or otherwise, and a game theoretic analysis can give much more robust performance guarantees than reliance on the honesty of certain users.
    \item \cite{SoKConsensus}: incentivization in committee-based blockchain consensus protocols (with leader) has started to see some study, but is far from mature. This area will benefit from combining formal economic and game theoretic analysis with cryptography.
    \item \cite{SOKGameTheoryBlockchain}:  
    \begin{itemize}
        \item Game theory is natural in the decision making of all the consensus nodes in the blockchain networks. 
        \item The blockchain consensus protocol is expected to be incentive compatible.
    \end{itemize}
    \item \cite{SelfishMining}: Since Bitcoin mining is open to the public, oﬀering ﬁnancial rewards, we conjecture that altruistic miners are few.
    \item \cite{FruitChains}: Assuming honest participation, however, is a strong assumption, especially in a setting where honest players are expected to perform a lot of work.
    \item \cite{Fairledger}:  We have to take into account that every entity may behave rationally, and deviate from the protocol if doing so increases its benefit.
    \item \cite{Fairledger}: to prove that a protocol is correct in our model, we need to show that (1) the problem speciﬁcation is satisﬁed in case all the rational entities follow the protocol and there are at most f byzantine ones, and (2) following the protocol is an equilibrium for rational entities even in the presence of f byzantine ones.
    \item \cite{SoKToolsGameTheoryCryptocurrencies}:  having a system that is secure with some bounded number of Byzantine faults is not enough to have a decentralized system as decentralization cannot be assumed. Rather, incentives should be designed to ensure enough (honest) participation.
    \item \cite{Bitcoin}: As long as a majority of CPU power is controlled by nodes that are not cooperating to attack the network, they’ll generate the longest chain and outpace attackers.
    
\end{itemize}

==> RoughWork.tex <==
\section{RW}


\begin{lemma}\label{lem:boundedDeviatorBonus}
    In $\protocolName$, for any player $\playeri$ who decides on a value at height $\blockchainHeight> \initialisationHeight$, they receive a reward of $ \rewardHi < \frac{4}{3} \sharei^{\initialisationHeight} \rewardInitial$ for height $\blockchainHeight$.
\end{lemma}


\begin{proof}
    
    We can see that in $\protocolName$ the rewards for deciding on a value at height $\blockchainHeight$ are distributed at lines \ref{line:addReward} and \ref{line:splitDeviatorPot}. To prove that for any height $\blockchainHeight$, $\rewardHi < \frac{4}{3} \sharei^\initialisationHeight  \rewardInitial $ we will show that $ \shareHi \stakeHi < \sharei^{\blockchainHeight-1} \stakei^{\blockchainHeight-1}+ \frac{4}{3} \sharei^\initialisationHeight \cdot \rewardInitial$. 



    Let there be a set of players \textit{newDevs} controlling $\slashedShare$ at height $\blockchainHeight-1$ identified as deviating for the first time in the value at height $\blockchainHeight$. 
    This results in $\playeri$'s share being updated according to line \ref{line:adjustShares}, which implies $\shareHi =\frac{\sharei^{\blockchainHeight-1}}{1-\slashedShare}$. Furthermore, the new total reward for height $\blockchainHeight$ is $\reward^\blockchainHeight= (1-\slashedShare) \reward^{\blockchainHeight-1}  $ (line \ref{line:adjustReward}), while the total stake before distributing rewards for height $\blockchainHeight$ is adjusted to $(1-\slashedShare) \stake^{\blockchainHeight-1} $ (line \ref{line:adjustStake}). We then have to add the slash bonus of $\sum_{j \in \textit{newDevs}} \textit{Genesis.shares}()[j] \cdot \reward^\blockchainHeight$  (line \ref{line:splitDeviatorPot}) and the normal reward of $\reward^\blockchainHeight$  (line \ref{line:addReward}) to the total stake. 

    First observe that  
    \normalsize
    \begin{equation}
    \begin{split}
         \sharei^{\blockchainHeight} \reward^{\blockchainHeight} &= \frac{\sharei^{\blockchainHeight-1}}{1-\slashedShare} (1-\slashedShare) \reward^{\blockchainHeight-1}  \\ 
        &= \sharei^{\blockchainHeight-1}  \reward^{\blockchainHeight-1}.
    \end{split}
    \end{equation}
    
    This means $\sharei^{\blockchainHeight} \reward^{\blockchainHeight}= \sharei^\initialisationHeight \cdot \rewardInitial$ for all $\blockchainHeight \geq 1$.

    Next, notice that $\sum_{j \in \textit{newDevs}} \textit{Genesis.shares}()[j]$ must be less then $\partialSyncAdvLimit$. This is because the shares of players who remain in the protocol are lower-bounded by their initial shares (due to the increasing share adjustment at line \ref{line:adjustShares}), and the fact that a decision on any value requires players controlling more than $\partialSyncMajority$ to agree on a value (and as such, players who controlled less than $\partialSyncAdvLimit$ of the share at initialisation to disagree). 

    Putting this together gives a total stake at height $\blockchainHeight$ of:
   
    \begin{equation}
    \begin{split}
        \stake^{\blockchainHeight} &=(1-\slashedShare) \stake^{\blockchainHeight-1} \\
        & +\sum_{j \in \textit{newDevs}} \textit{Genesis.shares}()[j] \cdot  \reward^\blockchainHeight + \reward^\blockchainHeight \\
        &< (1-\slashedShare) \stake^{\blockchainHeight-1} + \frac{1}{3} \reward^\blockchainHeight + \reward^\blockchainHeight \\
        &= (1-\slashedShare) \big( \stake^{\blockchainHeight-1} +\frac{4}{3} \reward^{\blockchainHeight-1} \big).
    \end{split}
    \end{equation}
    
    Therefore $\playeri$'s stake at height $\blockchainHeight$, $\shareHi \stakeH $ can be described by the following inequality 
    
    \begin{equation}
    \begin{split}
        \shareHi \stakeH &<\shareHi (1-\slashedShare) \big( \stake^{\blockchainHeight-1} +\frac{4}{3} \reward^{\blockchainHeight-1} \big) \\ 
        &= \frac{\sharei^{\blockchainHeight-1} (1-\slashedShare)}{1-\slashedShare}  \big( \stake^{\blockchainHeight-1} +\frac{4}{3} \reward^{\blockchainHeight-1} \big) \\ 
        &= \sharei^{\blockchainHeight-1}  \big( \stake^{\blockchainHeight-1} +\frac{4}{3} \reward^{\blockchainHeight-1} \big).
    \end{split}
    \end{equation} 
    
    This implies $\playeri$'s reward for height $\blockchainHeight$ is less than $ \frac{4}{3} \ \sharei^{\blockchainHeight-1} \ \reward^{\blockchainHeight-1}$.
    From Equation \ref{eq:ConstantReward}, this implies $\playeri$ receives a reward of less than $\frac{4}{3} \sharei^\initialisationHeight  \rewardInitial$, as required.
\end{proof}

However, \cite{BlockchainWithoutWastePoS} provides some novel approaches to incentivisation in SMR protocols, and agree that in the tokenised setting, players must be incentivised to follow the protocol to guarantee SMR. This is extended in \cite{EvolutionOfSharesPoS} where it is demonstrated that if rewards are distributed in (expected) proportion to the amount of stake a player owns, and all players follow the protocol, bounds can be placed on player stake distribution over time. Again, the player model is restricted to only rational players. As rewards in \cite{EvolutionOfSharesPoS} are only paid fairly in expectancy, it is not possible to guarantee the fairness that we define in Definition \ref{def:fair}.



Therefore, rational players prefer to wait some number of rounds for messages to be delivered. A rational player $\playeri$ will have a perceived distribution, say with mean $\Delta_i$, of what the real delivery delta is at any given time given the responsiveness of all other players up until that point. If a statistically significant amount of rounds pass after $\Delta_i$ without progression towards a decision, it must be that some subset of players are out of synchrony with the network. As the maximum network delay $\Delta$ can be arbitrarily big, this implies the number of decisions that can be made instead of waiting for these players is $\Omega(\frac{\Delta}{\Delta_i})$. As such $\playeri$ will obey some timeout, and attempt to transition to the next epoch where decisions do not depend on this asynchronous subset of players. 


    $\playeri$ waits indefinitely for messages, and the proposer experiences a significantly larger message delivery delay than $\playeri$, then this message may never come. Therefore, $\playeri$ will choose some number of rounds $\timeouti>0$ as their timeout, after which they will progress to the next protocol step (lines \ref{line:tab:onTimeoutPropose}, \ref{line:tab:onTimeoutPrevote}, \ref{line:tab:onTimeoutPrecommit}). \label{proof:followSomeTimeout}
    
    Rational players are aware that there is a fixed, but unknown, upperbound $\Delta$ on message delivery between players in synchrony, which we refer to as $\Delta$-synchrony, but are unaware of how many players are in $\Delta$-synchrony at any given time.
    
    
    Now we must ensure rational players do not wait indefinitely for messages. 
    
    Recall that in Tenderstake, rational players are modelled as assuming for some unknown but fixed $\Delta$, they are in $\Delta$-synchrony with some subset of players.
    
    At any round $\round$, in order to calculate expected utility for some future round, $\playeri$ will have a private distribution of expected message delivery times from other players in synchrony\footnote{The distribution of expected message delivery times will be a function of some starting estimate at initialisation (perhaps based on a \textit{Genesis} suggested value, as in \cite{LatestGossipTendermint}), and the observed responsiveness of all other players up until round $\round$.}, and thus an expected number of decisions up until that future round. Let $\timeout^\round_i$ be such that according to $\playeri$'s private information, messages taking longer than $\timeout^\round_i$ are sent by players out of synchrony with $\playeri$ with statistical significance\footnote{This statistical significance can be with respect to a function $\negligible$, although rational players may perceive a higher utility by choosing a larger number. This optimisation is unnecessary for the proof.}. 
    
    If the subset of players in synchrony with $\playeri$, including $\playeri$, do not control more than $\partialSyncMajority $ of the total stake, $\playeri$ is indifferent to timing out, as no decision is possible. 
    Otherwise, consider the subset of players in synchrony with $\playeri$, including $\playeri$, controlling more then $\partialSyncMajority $ of the total stake. As messages sent by players out of synchrony with $\playeri$ take arbitrarily long to deliver, the number of decisions that can be made by using a timeout of $\timeout^\round_i$ and transitioning to a proposer in synchrony with $\playeri$ is arbitrarily large. Furthermore, as $\playeri$ is unaware of how many players are in synchrony with $\playeri$, the probability of that subset controlling more than $\partialSyncMajority $ of the stake will be positive. This implies $\playeri$ has positive expectancy to obey such a timeout $\timeout^\round_i$. Therefore, rational players obey some timeout, and will not wait indefinitely for messages. 
